Toward more accurate measurement of the impact of online instructional design on students' ability to transfer physics problem-solving skills

In two earlier studies, we developed a new method to measure students' ability to transfer physics problem solving skills to new contexts using a sequence of online learning modules, and implemented two interventions in the form of additional learning modules designed to improve transfer ability. The current paper introduces a new data analysis scheme that could improve the accuracy of the measurement by accounting for possible differences in students' goal orientation and behavior, as well as revealing the possible mechanism by which one of the two interventions improves transfer ability. Based on a two by two framework of self-regulated learning, students with a performance-avoidance oriented goal are more likely to guess on some of the assessment attempts in order to save time, resulting in an underestimation of the student populations' transfer ability. The current analysis shows that about half of the students had frequent brief initial assessment attempts, and significantly lower correct rates on certain modules, which we think is likely to have originated at least in part from students adopting a performance-avoidance strategy. We then divided the remaining population, for which we can be certain that few students adopted a performance-avoidance strategy, based on whether they interacted with one of the intervention modules designed to develop basic problem solving skills, or passed that module on their first attempt without interacting with the instructional material. By comparing to propensity score matched populations from a previous semester, we found that the improvement in subsequent transfer performance observed in a previous study mainly came from the latter population, suggesting that the intervention served as an effective reminder for students to activate existing skills, but fell short of developing those skills among those who have yet to master it.

==> Unused Content/discussion_original.tex <==
\section{Discussion}\label{sec:discussion}

% RQ1
We find that roughly half of the students either occasionally or frequently adopt learning strategies that are motivated by extrinsic value -- skipping their initial attempts on 2-4 of the first four modules.
Several types of behavior may result in a student having many Brief Attempts, such as randomly guessing on each first attempt in order to quickly access the IC or working on the problems together with other students and then copying the answer into their own account.

% RQ2
Extrinsic value-motivated learning strategies can sometimes have significant impact on the outcomes of measurement conducted in an online, self-regulated environment.
In this case, it leads to potential underestimation of students' true ability to transfer their problem solving skill from one module to the next, and masked the effectiveness of the intervention on a subgroup of students.
\textcolor{red}{[Talk about results from RQ2 analysis.]}
The fact that so many students simply quickly click through the initial attempt is a critical piece of information for researchers to consider when attempting to measure whether the inclusion of scaffolding modules (such as the on-ramp module, OLM 1 in Fig.~\ref{fig:design}) positively affects student problem-solving in subsequent modules.
If students do not seriously engage with the material, then it may not be reasonable to consider them as part of the treatment group when investigating the effects of new instructional material.

% RQ3
We observe in Fig.~\ref{fig:zigzag_matched_all} that the addition of the on-ramp module primarily improved student passing rates in 2018 over 2017 in the RK sequence (Fig.~\ref{fig:zigzag_matched_all:RK}), which was generally more difficult for students than the AM sequence (Fig.~\ref{fig:zigzag_matched_all}:AM).
This effect was less statistically significant in the earlier study~\cite{chen2019perc} because we did not consider students' learning strategy.
By further considering whether the 2018 students belong to the Pass On-Ramp Pre-study or Pass On-Ramp Post-study groups (Fig.~\ref{fig:zigzag_matched_onramp}), we find that the improvement in the RK sequence is primarily occurring among the Pass On-Ramp Pre-study students (Fig.~\ref{fig:zigzag_matched_onramp:RK_passInPre}), indicating that the main benefit of the on-ramp module is to facilitate the reminder effect.
However, our results cannot completely rule out the possibility of a learning effect.
Though the differences did not end up being statistically significant after $p$-adjustment (Table~\ref{tab:zigzag_p_adj}), we do observe in Fig.~\ref{fig:zigzag_matched_onramp:RK_passInPost} that the 2018 students perform somewhat better than the matched 2017 students in RK Example Pre-study and RK Example Post-study attempts.
We observe the same effect on AM Tutorial Pre-study and AM Example Pre-study attempts among Pass On-Ramp Pre-study students (Fig.~\ref{fig:zigzag_matched_onramp:AM_passInPre}).

Another possible interpretation is that the on-ramp module served as a sensitive filter in the current analysis, selecting those students who have better mastery of the basic concepts and are primed to benefit from the tutorial.
Using propensity score matching for the 2017 sample reduces the likelihood of the filtering effect being dominant, but the current form of propensity scores (based upon exam scores) cannot completely rule out this possibility.
As a result, our analysis only suggests that the on-ramp module is beneficial for a subsample of students who had prior knowledge before engaging with the OLM sequence, by reminding them of the basic skills necessary for solving the problems in the sequence.
It is unknown if it had any effect on other students, such as those who frequently adopted extrinsic value-motivated strategies, or who had weaker prior knowledge of the relevant physics concepts.

\subsection{Limitations}
The primary inherent limitation to studies of self-paced instructional material is that it is reliant upon student interaction with online learning modules.
This makes the collected clickstream data, especially of attempt durations, inherently noisy due to the possibility of students leaving a session open without actively working on the material.
Keeping this in mind, we only used short attempt durations as a measure, since attempts under a cutoff duration are not susceptible to these effects.
Another limitation of the current study is the use of exam scores as propensity scores.
More relevant propensity scores could potentially be generated from students' behavior and performance on similar OLMs that they accessed prior to engaging with the tutorial sequence.

\subsection{Conclusion}
Gathering data from online learning modules can be a rich source of information for investigating student learning.
Future studies could continue to develop additional modules and use or expand upon the techniques described here in order to test the effects of various instructional methods.
Studies could also incorporate additional information such as student demographic information and attitudes about physics (e.g., self-efficacy, perceived recognition, interest in physics, and physics identity) in order to investigate how inequities in physics education play out during problem-solving.
\textcolor{red}{Chen/Matt make sure to review these last two sentences and make sure you agree!}
Finally, the findings in this paper also suggest that self-paced learning tools may be most effective for students who have already been primed with the prerequisite knowledge to solve the problems (i.e., from in-class instruction).
However, these online learning modules can be a powerful supplement to in-class instruction that provide more flexibility for supplemental instruction than traditional homework problems.

==> Unused Content/discussion_outline.tex <==
Discussion outline

RQ1
    -We find that roughly half of the students are skipping their initial attempts on 2-4 of the first four modules.
    -Several types of behavior may result in a student having many Brief Attempts, such as randomly guessing on each first attempt or working on the problems together with other students and then copying the answer into their own account.

RQ2
    -The fact that so many students simply quickly click through the initial attempt is a critical piece of information for researchers to consider when attempting to measure whether the inclusion of scaffolding modules (such as the on-ramp module, OLM 1 in Fig.~\ref{fig:design}) positively affects student problem-solving in subsequent modules.
    -If students don't seriously engage with the material, then it may not be reasonable to consider them as part of the treatment group when investigating the effects of new instructional material.
    
RQ3
    -We observe in Fig.~\ref{fig:zigzag_matched_all} that the addition of the on-ramp module primarily improved student passing rates in 2018 over 2017 in the RK sequence (Fig.~\ref{fig:zigzag_matched_all:RK}), which was generally more difficult for students than the AM sequence (Fig.~\ref{fig:zigzag_matched_all}:AM).
    -By further considering whether the 2018 students belong to the Pass On-Ramp Pre-study or Pass On-Ramp Post-study groups (Fig.~\ref{fig:zigzag_matched_onramp}), we find that the improvement in the RK sequence is primarily occurring among the Pass On-Ramp Pre-study students (Fig.~\ref{fig:zigzag_matched_onramp:RK_passInPre}), indicating that the main benefit of the on-ramp module is to facilitate the reminder effect.
    -However, this is not to say that the learning effect was entirely absent. Though the differences did not end up being statistically significant after $p$-adjustment (Table~\ref{tab:zigzag_p_adj}), we do observe in Fig.~\ref{fig:zigzag_matched_onramp:RK_passInPost} that the 2018 students perform somewhat better than the matched 2017 students in RK Example Pre-study and RK Example Post-study attempts. We observe the same effect on AM Tutorial Pre-study and AM Example Pre-study attempts among Pass On-Ramp Pre-study students (Fig.~\ref{fig:zigzag_matched_onramp:AM_passInPre}).

Limitations
    -Reliant upon student interaction with online learning modules.
    -This makes data, especially with attempt durations, inherently noisy due to the possibility of students leaving a session open without actively working on the material.
    -Keeping this in mind, we only focus on using short attempt durations as a measure, since attempts under a cutoff duration are not susceptible to these effects.

Concluding thoughts & future directions
    -Gathering data from online learning modules can be a rich source of information for investigating student learning.
    -Future studies could continue to develop additional modules and use techniques such as those described here in order to test the effects of various instructional methods.
    -Studies could also incorporate additional information such as student demographic information and attitudes about physics (e.g., self-efficacy, perceived recognition, interest in physics, and physics identity) in order to investigate how inequities in physics education play out during problem-solving.

==> Unused Content/experiment_design.tex <==
% \tikzset{>=latex} %usually I like these arrowheads better, but with how short the arrow lines have become I think the default ones work better

%scale will change the scale of diagrammatic elements (lengths); the node style scale will change text size
\begin{tikzpicture}[scale=0.75, every node/.style={scale=0.75}]
	\tikzmath{
		\L = 2; %length of overall module side
		\sep = \L/24; %separation from outer rectangle to inner
		\ICh = 5*\L/9; %height of an IC box
		\ACh = 2*\L/9; %height of an AC box
		\arr = \L - \ICh - \ACh - 2*\sep; %arrow length
		\H = \L/4; %vertical separation between rows
	}
	\def\colormodulefill{white} %background fill color
	\def\colorAC{orange} %assessment border color
	\def\colorACfill{orange!10} %assessment fill color
	\def\colorIC{blue} %instruction color
	\def\colorICfill{blue!10} %instruction fill color
	\def\outerround{4pt} %rounding of outer rectangles
	\def\innerround{2pt} %rounding of inner rectangles
	\def\arrowround{1.5pt} %rounding of arrow lines (to/from modules 4A/4B)
	
	\coordinate (OLM1) at (0,\L+\H/2);
	\coordinate (OLM2) at ($(OLM1)+(\L+\arr,0)$);
	\coordinate (OLM3) at ($(OLM2)+(\L+\arr,0)$);
	\coordinate (OLM4) at ($(OLM3)+(\L+\arr,0)$);
% 	\coordinate (OLM4) at ($(OLM3)+(\L+2*\arr,0)$);
% 	\coordinate (OLM4A) at ($(OLM4)+(0,\L/2+\H/2)$);
% 	\coordinate (OLM4B) at ($(OLM4)+(0,-\L/2-\H/2)$);
% 	\coordinate (OLM5) at ($(OLM4)+(\L+2*\arr,0)$);
	\coordinate (OLM5) at ($(OLM4)+(\L+\arr,0)$);
	
	    %primary module drawing (sans instructional components) [modules 1 through 5]
	\foreach \modlabel/\modnum/\AC/\IC in {On-Ramp/1/1, Tutorial/2/2, Example 1/3/3, Example 2/4/4, Quiz/5/5}
	{
	        %outer rectangle
	    \draw[fill=\colormodulefill, rounded corners=\outerround] (OLM\modnum) rectangle ($(OLM\modnum) + (\L,\L)$);
	        %inner assessment rectangle
    	\draw[color=\colorAC, fill=\colorACfill, rounded corners=\innerround] ($(OLM\modnum)+(\sep,\L-\ACh-\sep)$) rectangle ($(OLM\modnum) + (\L-\sep, \L-\sep)$) node[black, opacity = 1, midway, align=center]{AC\AC};
    	    %arrows between instruction and assessment
    	\draw[->] ($(OLM\modnum)+(\L/4, \L-\sep-\ACh)$) --++ (0,-\arr);
    	\draw[->] ($(OLM\modnum)+(3*\L/4, \sep+\ICh)$) --++ (0,\arr);
    	    %module label
	    \node at ($(OLM\modnum)+(\L/2, \L+2*\sep)$) {\modlabel};   
	}
	    %instructional components [modules 1 through 4]
	\foreach \modnum/\IC in {1/Solution, 2/Tutorial, 3/Solution, 4/Solution}
	{
	        %inner instruction rectangle
    	\draw[color=\colorIC, fill=\colorICfill, rounded corners=\innerround] ($(OLM\modnum)+(\sep,\sep)$) rectangle ($(OLM\modnum) + (\L-\sep, \ICh+\sep)$) node[black, opacity = 1, midway, align=center]{IC\modnum:\\\IC};
	}
	    %draw the quiz instructional component separately since it has a different design (dashed, not filled)
	\draw[dashed, color=\colorIC, rounded corners=\innerround] ($(OLM5)+(\sep,\sep)$) rectangle ($(OLM5) + (\L-\sep, \ICh+\sep)$) node[black, opacity = 1, midway, align=center]{IC5:\\Empty};
	
	    %arrows connecting modules in sequence
		%OLM1 -> OLM2
	\draw[->, thick] ($(OLM1)+(\L, \L/2)$) --++ (\arr,0);
		%OLM2 -> OLM3
	\draw[->, thick] ($(OLM2)+(\L, \L/2)$) --++ (\arr,0);
		%OLM3 -> OLM4
	\draw[->, thick] ($(OLM3)+(\L, \L/2)$) --++ (\arr,0);
	    %OLM4 -> OLM5
	\draw[->, thick] ($(OLM4)+(\L, \L/2)$) --++ (\arr,0);
% 		%OLM3 -> OLM4A/B
% 	\draw[->, thick, rounded corners=\arrowround] ($(OLM3)+(\L, \L/2)$) --++ (\arr,0) --++ (0,\L/2+\H/2) --++(\arr,0);
% 	\draw[->, thick, rounded corners=\arrowround] ($(OLM3)+(\L, \L/2)$) --++ (\arr,0) --++ (0,-\L/2-\H/2) --++(\arr,0);
% 	    %OLM4A/B -> OLM5
% 	\draw[->, thick, rounded corners=\arrowround] ($(OLM4A)+(\L, \L/2)$) --++ (\arr,0) --++ (0,-\L/2-\H/2) --++(\arr,0);
% 	\draw[->, thick, rounded corners=\arrowround] ($(OLM4B)+(\L, \L/2)$) --++ (\arr,0) --++ (0,+\L/2+\H/2) --++(\arr,0);
	
% 	    %OLM4 dashed rectangle
% 	\draw[dashed, rounded corners=\outerround] ($(OLM4B) + (-\arr-\sep,-2*\sep)$) rectangle ($(OLM4A) + (\L+\arr+\sep,\L+4*\sep)$);
	
	    %notes specifying which modules were added in 2018
	\node at ($(OLM1) + (\L/2, \L+8*\sep)$) {\textit{Added in 2018}};
	\node at ($(OLM4) + (\L/2, \L+8*\sep)$) {\textit{Added in 2018}};
% 	\node[align=center] at ($(OLM2) + (\L/2, \L+10.5*\sep)$) {\textit{Common to}\\\textit{2017 and 2018}};
% 	\node[align=center] at ($(OLM3) + (\L/2, \L+10.5*\sep)$) {\textit{Common to}\\\textit{2017 and 2018}};
% 	\node[align=center] at ($(OLM5) + (\L/2, \L+10.5*\sep)$) {\textit{Common to}\\\textit{2017 and 2018}};
	
	\node[align=center] at ($(OLM3) + (\L/2, -\L/4)$) {
	%\textbf{M\#} = \textbf{M}odule \textbf{\#},
	\textbf{AC} = \textbf{A}ssessment \textbf{C}omponent \hspace{1cm}	\textbf{IC} = \textbf{I}nstructional \textbf{C}omponent
	};
\end{tikzpicture}

==> Unused Content/intro_original.tex <==
Studies in both general human problem solving and problem solving in physics have long shown that it is difficult for novices to transfer the understanding and skills learned in one problem context to a different, new context~\cite{Broudy1977, Detterman1993, Bransford1999}.
In physics, it is well known that novices tend to focus more on superficial differences between problems and pay less attention to deep structural similarities between problems~\cite{Chi1982}.
In an earlier study involving a sequence of three online learning modules, we observed that while most introductory-level college physics students learned to solve a specific problem after engaging with an online problem solving tutorial in the first module, student performance when solving similar problems on two subsequent modules was either unchanged or only slightly improved~\cite{chen2018perc}.
Following this, in another study we found evidence suggesting that the inclusion of an ``on-ramp'' module (a scaffolding module containing simpler problems using the physics concepts underpinning the subsequent modules) has a significant impact on students' performance on subsequent modules~\cite{chen2019perc}.
However, this study did not take into account the impact of different modes of engagement by students in a self-regulated online learning environment, nor did it provide insight into the mechanism by which the on-ramp module impacts downstream behavior.

Since the online learning modules are given to the students to complete at their own pace, we can turn to frameworks such as Boekaerts's~\cite{boekaerts2000} model of self-regulated learning (SRL) in order to gain insight into how students go about engaging with self-paced material.
Boekarts proposes that students will engage with SRL using one of two modes: a ``mastery mode'' and a ``coping mode.''
Students working in a mastery mode will seek out knowledge and skills to improve their mastery of the material, while those working in a coping mode will seek to preserve resources and avoid damage to their well-being (i.e., do the minimum necessary).
A related model is Pintrich's four-phase model of regulated learning~\cite{pintrich2000, pintrich2004}.
Pintrich describes how students use four categories of regulation -- cognition, motivation, behavior, and context -- throughout each of four phases of engagement in order to decide how to engage with the material~\cite{pintrich2000, pintrich2004}.
Pintrich's model is summarized succinctly by Winne~\cite{winne2015} as describing how a learner's motivation and achievement goal orientation influences their engagement.
The frameworks of Boekaerts~\cite{boekaerts2000} and Pintrich~\cite{pintrich2000, pintrich2004} are both helpful in understanding why students may choose not to engage with the material, and remind us that when researching the effects of self-paced learning tools it is important to take steps to check that the students gave themselves the opportunity to learn from the material.
In particular, we must check for students that are exhibiting an extrinsic value-oriented strategy of quickly skipping through the material in order to preserve resources while obtaining credit for the assignment.

We are further interested in the mechanism by which the on-ramp module can improve subsequent performance.
Among those students who seriously engage with the material and solve the scaffolding problem in the on-ramp module, there will be some who began the sequence of online learning modules already equipped with the requisite knowledge to solve the problems, and for these students the on-ramp module will provide a ``reminder effect,'' where the students are reminded of their prior knowledge and primed to use that knowledge in subsequent assessments.
Other students may need additional instruction before solving the problems, and so will initially struggle with the scaffolding problem but be able to solve it after viewing some instructional material, an effect we will refer to as the ``learning effect.''

\begin{enumerate}[label={\bfseries RQ\arabic*}, topsep=5pt, itemsep=0pt]
  %RQ0 (unstated): Does the addition of a scaffolding problem increase student performance in subsequent low-stakes online assessments?
  \item \label{rq:behavior} Do students employ different learning strategies when interacting with the online learning modules (e.g., seriously attempting the problem before instruction or skipping through to the instructional content before seriously attempting the problem)?
  \item \label{rq:engagement} How does an extrinsic value-oriented strategy employed by students affect the assessment of learning and transfer in an online environment, and how can we mitigate this?
  \item \label{rq:onramp} By what mechanism do the on-ramp modules improve subsequent performance (i.e., by reminding students of previously learned material or by teaching students new skills)?
\end{enumerate}

==> Unused Content/results_original.tex <==
% RQ1: \label{rq:behavior} Do students employ different learning strategies when interacting with the online learning modules (e.g., seriously attempting the problem before instruction or skipping through to the instructional content before seriously attempting the problem)?

In order to investigate whether the student OLM records can be used to select those students who are seriously engaging with the material and answer \ref{rq:behavior}, we can consider the students by their number of Brief Attempts (Table~\ref{tab:2018_BA_groups}).
The sample of students can be roughly split in half based on the number of brief attempts used during the first four modules.
We see that roughly half of the students have zero to one Brief Attempts while the remaining half of students have two or more Brief Attempts throughout the first four modules.
This is indicative of an extrinsic value-oriented strategy, where students quickly skip through the required initial attempt by submitting a guess in order to access the instructional material in the IC before solving the problem post-instruction.
Figure~\ref{fig:zigzag_BA} shows the pass rates of students who have 0-1, 2-3, or 4 Brief Attempts throughout the OLM sequence.
These pass rates are shown separately for the RK sequence (Fig.~\ref{fig:zigzag_BA:RK}) and AM sequence (Fig.~\ref{fig:zigzag_BA:AM}).

In both Fig.~\ref{fig:zigzag_BA:RK} and Fig.~\ref{fig:zigzag_BA:AM}, students in the 0-1 Brief Attempts group often slightly outperform those in the 2-3 Brief Attempts group, although the only modules in which this difference in pass rates is statistically significant according to Fisher's exact test are the Example Pre-study attempts on both the RK sequence ($p = 0.001$) and the AM sequence ($p < 0.001$) as well as the RK Tutorial Post-study ($p = 0.029$) and RK Example Post-study ($p = 0.018$) attempts.
The 4 Brief Attempts groups on each OLM sequence behave somewhat erratically, likely due to their non-standard engagement with the material since their first attempt on each non-Quiz module lasts less than 35 seconds.

% RQ2: \label{rq:engagement} How does an extrinsic value-oriented strategy employed by students affect the assessment of learning and transfer in an online environment, and how can we mitigate this?

Since in most cases the pass rates of the students in different Brief Attempt groups is indistinguishable, the answer to \ref{rq:engagement} is that success rates alone are insufficient to distinguish which students are seriously engaging with the problem before submitting an answer.
Additional information, such as the duration of the attempt, is necessary in order to identify a subsample of students whose Pre-study attempts could have reasonably been serious efforts to solve the problem.
\textcolor{red}{Does this need more for RQ2? It's difficult to talk about this RQ much in the results section since it's largely a synthesis of the implications of RQ1.}


% RQ3: \label{rq:onramp} By what mechanism do the on-ramp modules improve subsequent performance (i.e., by reminding students of previously learned material or by teaching students new skills)?
Since many students will not have seriously engaged with the material during their initial attempt, we limited our sample to only those students with 0-1 Brief Attempts in either 2017 or 2018 in order to investigate the effect of the on-ramp module and answer \ref{rq:onramp}.
As discussed in Section~\ref{subsec:analysis}, we used propensity score matching in course exam scores in order to obtain matching subsamples of the 2017 students to the 2018 students.
Figure~\ref{fig:zigzag_matched_all} shows the pass rates of the 2018 students with 0-1 Brief Attempts along with the matched subsample of 2017 students in both the RK (Fig.~\ref{fig:zigzag_matched_all:RK}) and AM (Fig.~\ref{fig:zigzag_matched_all:AM}) sequences.
In the RK sequence (Fig.~\ref{fig:zigzag_matched_all:RK}), we see that the 2018 students, who were given the additional on-ramp module prior to the tutorial module, outperformed the matched 2017 students in their RK Tutorial Pre, RK Example Pre, and RK Example Post-study attempts.
Each of these three improvements is statistically significant (see the first row of Table~\ref{tab:zigzag_p_adj}), while the pass rates in RK Tutorial Post-study and the RK Quiz are not statistically significantly different.
However, in the AM sequence (Fig.~\ref{fig:zigzag_matched_all:AM}), we see no statistically significant differences in any module (second row of Table~\ref{tab:zigzag_p_adj}).
This is perhaps due to a ceiling effect, with little room for improvement over the 2017 students with the inclusion of the on-ramp module.

==> Unused Content/table_olm_BA_groups.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{r r | C{17mm} C{17mm} C{12mm} C{12mm}}
            & Brief     & Pass Before   & Pass After    & \multirow{2}{*}{Fail} & \multirow{2}{*}{Total} \\
            & Attempts  & Study         & Study         &                       & \\
            \hline
            \multirow{3}{*}{RK}
            & 0-1       & 32            & 57            & 11                    & 100 \\
            & 2-3       & 20            & 42            & 20                    & 82 \\
            & 4         & 2             & 7             & 7                     & 16 \\
            \hline
            \multirow{3}{*}{AM}
            & 0-1       & 32            & 47            & 12                    & 91 \\
            & 2-3       & 28            & 28            & 15                    & 71\\
            & 4         & 8             & 12            & 7                     & 27
    \end{tabular}
    \caption{The number of 2018 students in each OLM sequence and group by their number of Brief Attempts.
    Students are grouped into those who had 0-1 brief attempts, 2-3 brief attempts, and 4 brief attempts.}
    % \label{tab:2018_BA+onramp_groups}
\end{table}

==> Unused Content/table_unadjusted_p_values.tex <==
%table of unadjusted p-values, unlikely to keep in paper
\begin{table}[t] 
    \centering
    \begin{tabular}{c | c c c c c}
                & Tutorial  & Tutorial  & Example   & Example   & \multirow{2}{*}{Quiz} \\
        Fig.    & Pre       & Post      & Pre       & Post      & \\
        \hline
        \ref{fig:zigzag_matched_all:RK}
                & 0.009     & 0.132     & $<0.001$  & 0.002     & 0.120 \\
        \ref{fig:zigzag_matched_all:AM}
                & 0.336     & 0.094     & \textcolor{red}{0.044}     & 0.120     & \textcolor{red}{0.018} \\
        \ref{fig:zigzag_matched_onramp:RK_passInPre}
                & 0.001     & 1.000     & $<0.001$  & 0.005     & 0.289 \\
        \ref{fig:zigzag_matched_onramp:RK_passInPost}
                & 0.531     & 1.000     & 0.052     & 0.198     & \textcolor{red}{0.029} \\
        \ref{fig:zigzag_matched_onramp:AM_passInPre}
                & 0.603     & 0.355     & 0.053     & 0.492     & 0.103 \\
        \ref{fig:zigzag_matched_onramp:AM_passInPost}
                & 1.000     & 1.000     & 1.000     & 0.495     & 1.000
    \end{tabular}
    \caption{A list of $p$-values from Fisher's exact test comparing the performance of 2018 students and matched 2017 students on each assessment in the listed figure.
    }
    % \label{tab:zigzag_p_unadj}
\end{table}
